HomeSafe-Bench: Evaluating Vision-Language Models on Unsafe Action Detection for Embodied Agents in Household Scenarios

The rapid evolution of embodied agents has accelerated the deployment of household robots in real-world environments. However, unlike structured industrial settings, household spaces introduce unpredictable safety risks, where system limitations such as perception latency and lack of common sense knowledge can lead to dangerous errors. Current safety evaluations, often restricted to static images, text, or general hazards, fail to adequately benchmark dynamic unsafe action detection in these specific contexts. To bridge this gap, we introduce HomeSafe-Bench, a challenging benchmark designed to evaluate Vision-Language Models (VLMs) on unsafe action detection in household scenarios. HomeSafe-Bench is contrusted via a hybrid pipeline combining physical simulation with advanced video generation and features 438 diverse cases across six functional areas with fine-grained multidimensional annotations. Beyond benchmarking, we propose Hierarchical Dual-Brain Guard for Household Safety (HD-Guard), a hierarchical streaming architecture for real-time safety monitoring. HD-Guard coordinates a lightweight FastBrain for continuous high-frequency screening with an asynchronous large-scale SlowBrain for deep multimodal reasoning, effectively balancing inference efficiency with detection accuracy. Evaluations demonstrate that HD-Guard achieves a superior trade-off between latency and performance, while our analysis identifies critical bottlenecks in current VLM-based safety detection.

==> pics/anno_severity_table.tex <==
\begin{table}[htbp]
\centering
\footnotesize % 此表文字最密，建议用 footnotesize
\caption{Danger Categories and Severity Assessment}
\label{tab:severity}
\begin{tabularx}{\textwidth}{@{} l l l X @{}}
\toprule
\textbf{Cat.} & \textbf{Type} & \textbf{Severity} & \textbf{Criteria (Personal Injury / Economic Loss)} \\ \midrule
\multirow{4}{*}{\textbf{C1--C3}} & \multirow{4}{*}{\makecell[l]{Cutting, Blunt,\\Fire, Elec.}} & \textbf{L1 (Minor)} & Treated and released; superficial abrasions. \\
 & & \textbf{L2 (Mod.)} & Requires medical treatment (suturing, immobilization). \\
 & & \textbf{L3 (Severe)} & Hospitalization required; potential permanent damage. \\
 & & \textbf{L4 (Crit.)} & Life-threatening; fatality or irreversible trauma. \\ \midrule
\multirow{4}{*}{\textbf{C4}} & \multirow{4}{*}{\makecell[l]{Object / Env.\\Damage}} & \textbf{L1} & Economic loss < 100 RMB. \\
 & & \textbf{L2} & 100 -- 1,000 RMB. \\
 & & \textbf{L3} & 1,000 -- 10,000 RMB. \\
 & & \textbf{L4} & > 10,000 RMB. \\ \bottomrule
\end{tabularx}

\end{table}

==> pics/frame_overview.tex <==
\begin{figure}[t]
\centering

\includegraphics[width=\linewidth]{pics/abcd.pdf}

\caption{\textbf{Overview of HomeSafe-Bench and HD-Guard.} (a) Static vs. dynamic safety: Unlike static scenarios, domestic environments require continuous perception of dynamic physical hazards to prevent irreversible harm. (b) Data examples from HomeSafe-Bench: HomeSafe-Bench evaluates VLMs on unsafe action detection for household agents, with multi-dimensional annotations for immediate and latent hazards. (c) HD-Guard framework: A hierarchical streaming system coordinating FastBrain and SlowBrain to meet stringent latency constraints for real-world deployment. (d) Experimental results: Evaluations on HomeSafe-Bench highlight existing VLMs' limitations in danger detection.}
\label{fig:main}
\vspace{-0.6cm} 
\end{figure}

==> pics/label_align_lisan.tex <==
\begin{table}[htbp][t]
\centering
\caption{Inter-annotator agreement on categorical fields.
  $\kappa$: Cohen's $\kappa$ (unweighted for nominal fields;
  linear-weighted for ordinal fields marked with $\dagger$).
  Evaluated on the both-valid subset ($N=235$) except
  \textit{is\_valid} which uses all co-annotated videos ($N=412$).}
\label{tab:iaa_categorical}
\begin{tabular}{llccc}
\toprule
Field & Type & $N$ & Accuracy & $\kappa$ \\
\midrule
\textit{is\_valid}           & Binary  & 412 & 0.757 & 0.429 \\
\midrule
\textit{danger\_type}        & Nominal & 235 & 0.362 & 0.150 \\
\textit{severity}$^\dagger$  & Ordinal & 235 & 0.472 & 0.362 \\
\textit{reasoning\_difficulty}$^\dagger$ & Ordinal & 235 & 0.723 & 0.649 \\
\bottomrule
\end{tabular}
\end{table}

==> pics/table_benchmark_comparison.tex <==
\begin{table*}[t]
\centering
\label{tab:benchmark_comparison}
\caption{Comparison of HomeSafe-Bench with existing benchmarks.}
\resizebox{\textwidth}{!}{
\fontfamily{ptm}\selectfont
\begin{tabular}{lcccccccc} % 总共 9 列
\toprule
\multirow{2}{*}{Benchmark} & \multirow{2}{*}{\begin{tabular}{@{}c@{}}\# Test \\ Cases\end{tabular}} & \multicolumn{3}{c}{Modality} & \multicolumn{2}{c}{Data Source} & \multirow{2}{*}{\begin{tabular}{@{}c@{}}Customized \\ Scene\end{tabular}} & \multirow{2}{*}{\begin{tabular}{@{}c@{}}Decoupled \\ Evaluation\end{tabular}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-7}
 & & Video & Image & Audio & Simulation & Generative & & \\
\midrule
SafePlan-Bench~\cite{huang2025frameworkbenchmarkingaligningtaskplanning}
 & 2027 & $\times$     & $\times$     & $\times$     & $\times$     & $\times$     & $\times$ & $\checkmark$ \\
MSSBench~\cite{zhou2025multimodalsituationalsafety}  & 380 & $\times$     & $\checkmark$ & $\times$     & $\times$     & $\times$     & $\times$ & $\checkmark$ \\
ASIMOV-v2~\cite{jindal2025aiperceivephysicaldanger}  & 287 & $\checkmark$ & $\checkmark$ & $\times$     & $\times$     & $\times$     & $\checkmark$ & $\checkmark$ \\
IS-Bench~\cite{lu2025isbenchevaluatinginteractivesafety}  & 388 & $\checkmark$ & $\checkmark$ & $\times$     & $\checkmark$ & $\times$     & $\checkmark$ & $\times$ \\
\midrule
\textbf{HomeSafe-Bench}   & 438 & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
\bottomrule
\end{tabular}
}
\end{table*}

